Stochastic reconstruction of multiphase composite microstructures using statistics-encoded neural network for poro/micro-mechanical modelling

Understanding microstructure-property relationships (MPRs) is essential for optimising the performance of multiphase composites. Image-based poro/micro-mechanical modelling provides a non-invasive approach to exploring MPRs, but the randomness of multiphase composites often necessitates extensive 3D microstructure datasets for statistical reliability. This study introduces a cost-effective machine learning framework to reconstruct numerous virtual 3D microstructures from limited 2D exemplars, circumventing the high costs of volumetric microscopy. Using feedforward neural networks, termed the statistics-encoded neural network (SENN), the framework encodes 2D morphological statistics and infers 3D morphological statistics via a 2D-to-3D integration scheme. Statistically equivalent 3D microstructures are synthesised using Gibbs sampling. Hierarchical characterisation enables seamless capture of features across multiple scales. Validation on three composites demonstrates strong statistical equivalence between reconstructed and reference microstructures, confirmed by morphological descriptors and simulated macroscopic properties (e.g., stiffness, permeability). The SENN-based framework is a high-fidelity tool for efficiently and accurately reconstructing multiphase microstructures.

==> Makefile <==
DOC= data-driven-rom
LATEX=latex
PDFLATEX=pdflatex
BIBTEX=bibtex

\textbf{}
default: full

la:
	${LATEX} ${DOC}.tex
	dvips ${DOC}.dvi
	ps2pdf ${DOC}.ps

bib:
	${BIBTEX} ${DOC}

full: la bib
	make la la bib
	make la


